Tight Rates for Bandit Control Beyond Quadratics

Unlike classical control theory, such as Linear Quadratic Control (LQC), real-world control problems are highly complex. These problems often involve adversarial perturbations, bandit feedback models, and non-quadratic, adversarially chosen cost functions. A fundamental yet unresolved question is whether optimal regret can be achieved for these general control problems. The standard approach to addressing this problem involves a reduction to bandit convex optimization with memory. In the bandit setting, constructing a gradient estimator with low variance is challenging due to the memory structure and non-quadratic loss functions. In this paper, we provide an affirmative answer to this question. Our main contribution is an algorithm that achieves an $\tilde{O}(\sqrt{T})$ optimal regret for bandit non-stochastic control with strongly-convex and smooth cost functions in the presence of adversarial perturbations, improving the previously known $\tilde{O}(T^{2/3})$ regret bound from (Cassel and Koren, 2020. Our algorithm overcomes the memory issue by reducing the problem to Bandit Convex Optimization (BCO) without memory and addresses general strongly-convex costs using recent advancements in BCO from (Suggala et al., 2024). Along the way, we develop an improved algorithm for BCO with memory, which may be of independent interest.

==> backup.tex <==
\section{Backup}
In this work, we study the problem of online non-stochastic control with bandit feedback. This problem may be seen through the lens of a controller interacting with an environment evolving according to a time invariant linear dynamical system:
\begin{align}
\label{eq:lds}
x_{t+1}=Ax_t+Bu_t+w_t.
\end{align}
In this model, $A,B$ are the dynamics governing the system. $x_t, u_t, w_t$ are the state of the system, the control exerted to the system, and the perturbation affecting the system at time $t$, respectively. At time $t$, the controller observes the system's state $x_t$ and chooses a control $u_t$, to which they suffer some cost $c_t(x_t,u_t)$ depending on the state and control of the current step. The system then evolve according to Eq.~(\ref{eq:lds}) to reach the next state $x_{t+1}$. The works in non-stochastic control have caught much attention in the machine learning community in recent years \textcolor{red}{[cite]} and differ from the classical control problems \textcolor{red}{[cite]} in the relaxation of two standard assumptions in the latter: (1) the cost function $c_t$ can be time varying, adversarially chosen, and unknown a priori to the controller; (2) the perturbation $w_t$ does not need to follow some specified distribution and can be adversarially chosen as long as they are bounded \textcolor{red}{[cite]}. The natural performance metric under these relaxed assumptions is \textit{regret}, i.e. the excessive cost incurred by the controller over some time horizon comparing the cost incurred by the best control policy in some benchmark policy class $\Pi$, formally defined as
\begin{align*}
\regret_T(\texttt{controller})=\sum_{t=1}^T c_t(x_t,u_t)-\min_{\pi\in\Pi}\sum_{t=1}^T c_t(x_t^{\pi},u_t^{\pi}),
\end{align*}
where $(x_t,u_t)$ is the state-control pair reached by executing the controller at time $t$, and $(x_t^{\pi},u_t^{\pi})$ is the state-control pair reached by executing control policy $\pi$ at time $t$.

The question of interest in this work is the following: when is optimal rate possible in non-stochastic control under bandit feedback? 

Several previous works have made progress towards understanding this problem. Until recently any hope of obtaining optimal rate in bandit non-stochastic control relies on the assumption that the costs are strongly convex and smooth, and the perturbation sequence $\{w_t\}_{t=1}^T$ contains a stochastic component with a known lower bound on its covariance matrix~\citep{cassel2020bandit,sun2024optimal}. The recent advancement of \citep{suggala2024second} showed for the first time that optimal regret is achievable for strongly convex and smooth quadratic costs in the presence of adversarial perturbations. This work resolves the gap between upper and lower bounds in bandit control of LQR/LQG systems. It is left as an open question by \cite{suggala2024second} about whether similar results can be achieved beyond quadratic costs.  In this work, we answer this question affirmatively. 

\textcolor{purple}{Foster and Simchowitz 2020 showed that $\log T$ regret for full information control is possible. However, ``We note, however, that our approach heavily leverages the structure of linear con- trol with strongly convex, quadratic costs. We refer the to the related work section for discussion of further structural assumptions that facilitate logarithmic regret.'' }




Ideally, we want to develop $O(\sqrt{T})$ regret upper bound for bandit non-stochastic control problem with general convex cost functions. 

\begin{itemize}
\item \textbf{On extension and restarts}: non-stochastic control problems are in nature improper. Therefore, we probably don't need to use extension to make things proper. However, \cite{lattimore2024bandit} is still relevant since for adversarial costs we probably will need to consider restart. \textcolor{red}{It is also unclear how restart would be incorporated into the with-memory setting.}

\item \textbf{Memory structure}: Due to the negative result in \cite{suggala2024second}, the special memory structure in control problems has to be used to get $O(\sqrt{T})$ regret. In particular, the with-memory cost function induced by a control cost and its induced unary form exhibit the following structure:
\begin{align}
\label{eq:affine-memory}
f_t(x_{t-m+1:t})=\ell_t\left(B_t+\sum_{i=0}^{m-1}G^{[i]}Y_{t-i}x_{t-i}\right), \ \ \
\bar{f}_t(x)=\ell_t\left(B_t+\sum_{i=0}^{m-1}G^{[i]}Y_{t-i}x\right). 
\end{align}
When $\ell_t$ is strongly convex and smooth quadratic like the LQR/LQG setting considered in \cite{suggala2024second}, with the additional information of $G_t=\sum_{i=0}^{m-1}G^{[i]}Y_{t-i}$ available in the control problem, we can upper and lower bound $\nabla^2\bar{f}_t$ effectively. \textcolor{red}{However, for general convex control cost functions, it is unclear how this information can be used.} 

\item \textbf{Sampling scheme and high-dimensional estimator}: Quadratic cost functions were considered in \cite{suggala2021efficient}, \cite{sun2024optimal}, and \cite{suggala2024second} due to the possibility to find an unbiased/low-biased gradient/Hessian estimator for the with-memory cost function. In particular, the Cartesian product of spheres is no longer a sphere. Other suboptimal bounds in \cite{cassel2020bandit} and \cite{gradu2020non} used spherical sampling. \textcolor{red}{It is unclear what sampling mechanism is needed to hope for an $O(\sqrt{T})$ upper bound for general convex costs. We might want to use an ellipsoidal sampling scheme to effectively use the curvature information.}
\begin{itemize}
\item \cite{gradu2020non}: Showed that the unbiased gradient in no-memory case is unbiased for $\nabla f_t(x_{t-m+1},\dots,x_t)$ if $f_t$ is linear. Then, they use a linear approximation $\bar{f}_t$ of $f_t$ to bound the bias. The bias is of order $\delta\beta$. This approach does not seem to work if we use an ellipsoidal sampling scheme. 
\item \cite{cassel2020bandit}: Somehow without smoothness, the BCO-M in this paper still guarantees sublinear regret (the same rate $\tilde{O}(T^{3/4})$ as in \cite{gradu2020non}). Some notes on the techniques used in \cite{cassel2020bandit}: \textcolor{blue}{This method circumvents the estimator bias problem over the space of Cartesian product of unit spheres.}
\begin{itemize}
\item Previous work in general OCO-M to OCO problems all rely on the techniques developed in \cite{anava2015online}. The idea is to bound $|f_t(x_{t-m+1:t})-\bar{f}_t(x_t)|$ via regularity of the cost functions. 
\item \cite{cassel2020bandit} updates function every $H$ steps to decorrelate neighboring iterates (line 7 in Algorithm 2): The algorithm draws $b_t\sim\mathrm{Ber}(1/m)$ every round and updates only when $b_t=1$ and $b_{t-m+1}=\dots=b_{t-1}=0$. 
\begin{center}
\vspace{3mm}
\fbox{%
  \begin{minipage}{0.8\textwidth}
    ``The induced spacing between consecutive updates serves two purposes: first, it reduces the memory cost functions to functions of a single argument; second, it facilitates (conditional) probabilistic independence between consecutive updates."
  \end{minipage}
}
\vspace{3mm}
\end{center}
\item Direct application of Theorem 9 in \cite{cassel2020bandit} on Algorithm 1 in \cite{suggala2024second} does not work as $\nu_t=\|y_t-x_t\|_2$ is bounded by $O(1)$. Although the theoretical reduction does not directly apply, the method still may work (need to bound the exploration cost and the movement cost carefully using $\kappa$-convexity). 
\end{itemize}
\end{itemize}
\end{itemize}

\subsection{Small, potentially workable cornerstones}
\begin{itemize}
\item \textbf{Strongly convex and smooth control costs}: In this case, the affine memory structure still effectively gives us upper/lower bound on $\nabla^2\bar{f}_t$, i.e. $\bar{f}_t$ is $\kappa$-convex. Restart condition is also not needed. The only question to consider is the sampling mechanism. 
\textcolor{blue}{Note that this is not trivial since the induced unary form is not strongly convex.} \textcolor{red}{We need to restrict strong convexity and smoothness locally: unclear whether there exist other meaning function class other than quadratics satisfies strong convexity and smoothness globally.} \textcolor{blue}{See Section~\ref{sec:strongly-convex-and-smooth}.}
\end{itemize}

\paragraph{Main idea.} The idea is to combine the algorithmic techniques in \cite{suggala2024second} (to utilize and handle $\kappa$-convexity induced by strongly convex and smooth costs) and \cite{cassel2020bandit} (to reduce to no-memory BCO to circumvent the high-dimensional estimator problem beyond quadratics). 

When $\ell_t$ is strongly convex and smooth quadratic like the LQR/LQG setting considered in \cite{suggala2024second}, with the additional information of $G_t=\sum_{i=0}^{m-1}G^{[i]}Y_{t-i}$ available in the control problem, we can upper and lower bound $\nabla^2\bar{f}_t$ effectively. \textcolor{red}{However, for general convex control cost functions, it is unclear how this information can be used.} 

\paragraph{On loss functions.} We make the following assumptions on the sequence of loss functions. 
\begin{itemize}
\item \textbf{Affine memory structure}: $f_t:(\mathbb{R}^d)^m\rightarrow \mathbb{R}_+$ satisfies Eq.~\ref{eq:affine-memory} with $B_t\in\mathbb{R}^n, G^{[i]}\in\mathbb{R}^{n\times p}, Y_{t-i}\in\mathbb{R}^{p\times d}$. Denote $G_t=\sum_{i=0}^{m-1}G^{[i]}Y_{t-i}\in\mathbb{R}^{n\times d}$, and
$H_t=G_t^{\top}G_t\in\mathbb{R}^{d\times d}$.
\item \textbf{Curvature}: $\ell_t:\mathbb{R}^{n}\rightarrow \mathbb{R}_+$ and $\alpha I_{n}\preceq\nabla^2\ell_t(z)\preceq\beta I_{n}$, $\forall z\in\phi_t((\K+\mathbb{B}_{d})^m)$, where $\phi_t:(\mathbb{R}^d)^m\rightarrow\mathbb{R}^n$ denotes the transformation $(x_{t-m+1},\dots,x_t)\mapsto B_t+\sum_{i=0}^{m-1}G^{[i]}Y_{t-i}x_{t-i}$.
\item \textbf{Regularity}: Assume that for some convex set $\K$, $f_t(z_1,\dots,z_m)\le B$ and $\|\nabla f_t(z_1,\dots,z_m)\|_2\le G$, $\forall z_1,\dots,z_m\in\K+\mathbb{B}_{d}$. The convex set $\K$ has Euclidean diameter $D$.
\item \textbf{Induced unary form}: $\bar{f}_t:\mathbb{R}^d\rightarrow\mathbb{R}_+$ is given by $\bar{f}_t(z)=f_t(z,\dots,z)$. Note that $\bar{f}_{t}$ is $\kappa$-convex with $\kappa=\frac{\beta}{\alpha}$: $\alpha H_t\preceq \nabla^2\bar{f}_t(z)\preceq \beta H_t$, $\forall z\in\mathbb{R}^d$. 
\end{itemize}

\section{Proof of \cref{lem:control-reduction}}

In this section, we prove \cref{lem:control-reduction}. We begin by defining the Markov operator~\citep{simchowitz2020improper}. 

\begin{definition} [Markov operator]
\label{def:markov}
Given a partially observable LDS instance parametrized by dynamics $A\in\mathbb{R}^{d_x\times d_x}, B\in\mathbb{R}^{d_x\times d_u}, C\in\mathbb{R}^{d_y\times d_x}$ satisfying \cref{asm:strong-stabilizability} with $(\kappa, \gamma)$-strongly stabilizing $K$, define the Markov operator to be a sequence of matrices $G=\{G^{[i]}\}_{i\in\mathbb{N}}$ such that $\forall i\in\mathbb{N}$, $G^{[i]}$ is given by
\begin{align*}
G^{[i]}=\begin{bmatrix}
C \\
KC
\end{bmatrix}
(A+BKC)^{i-1}B\in\mathbb{R}^{(d_y+d_u)\times d_u}.
\end{align*}
\end{definition}

The next observation (\cref{obs:signal-obs}) relates $y_t(K)$, the signals used by the DRC policies (\cref{def:drc}), to the observations and controls along the learner's trajectory. This justifies the accessibility of the signals. 

\begin{observation}
\label{obs:signal-obs}
Given a partially observable LDS instance with $(\kappa, \gamma)$-strongly stabilizing $K$, let $G$ be the Markov operator in \cref{def:markov}.
For $t, m\in\mathbb{N}$, let $M_1,\dots,M_{t-1}\in\mathbb{R}^{m\times d_u \times d_y}$ be $(t-1)$ DRC matrices (\cref{def:drc}). Let $(y_t, u_t)$ be the observation-control pair reached by playing $M_1,\dots,M_{t-1}$ for time step $t=1,\dots, t-1$. Let $u_t(K)$ be the control at time $t$ by executing the linear policy $K$, i.e. $y_t(K)=Ku_t(K)$, and $y_t(K)$ be the would-be observation had $K$ been executed from the beginning of the time. Then, $(y_t,u_t)$ and $(y_t(K),u_t(K))$ can be related by the following equality:
\begin{align}
\label{eq:signal-obs}
\begin{bmatrix}
y_t\\
u_t
\end{bmatrix}=\begin{bmatrix}
y_t(K)\\
Ky_t(K)
\end{bmatrix}+\sum_{i=1}^t G^{[i]}\left(\sum_{j=0}^{m-1}M_{t-i}^{[j]}y_{t-i-j}(K)\right). 
\end{align}
In particular, \cref{eq:signal-obs} implies that $y_t(K)$ can be computed by the learner through access to the Markov operator $G$ and the observations along the learner's own trajectory.
\end{observation}

With \cref{eq:signal-obs}, we are almost ready to reduce the control instance to the BCO-M problem. One delicate detail is that the BCO-M problem is defined for vector-valued decisions, and the the space $\M(m,R_{\M})$ is a space of sequences of matrices. For clarity of presentation, we define the following embedding operators. 

\begin{definition} [Embedding operators]
\label{def:embed-op}
For $m, d_y, d_u\in\mathbb{N}$, denote $d=md_yd_u$. The embedding operator $\embed:(\mathbb{R}^{(d_u\times d_y)})^m\rightarrow\mathbb{R}^d$ is the natural embedding of a DRC controller $M=M^{[0:m-1]}$ (\cref{def:drc}) in $\mathbb{R}^d$. In particular, $\forall k\in[m-1],i\in[d_u],j\in[d_y]$,
\begin{align*}
\langle e_{kd_ud_y+(i-1)d_y+j}, \embed(M)\rangle = M^{[k]}_{ij}.
\end{align*}
Let $\embed_y:(\mathbb{R}^{d_y})^m\rightarrow \mathbb{R}^{d_u\times d}$ be given by $\forall y_{t-m+1},\dots,y_t\in\mathbb{R}^{d_y}$, $\forall i\in[d_u], k\in[m]$,
\begin{align*}
[\embed_y(y_{t-m+1:t})]_{i,j+1:j+d_y}=y_{t-k+1}, \ \ \ \text{if} \ \ \ j=(k-1)d_ud_y+(i-1)d_y.
\end{align*}
\end{definition}

\begin{proof} [Proof of \cref{lem:control-reduction}]
Let $B_t=(y_t(K), Ky_t(K))+\sum_{i=m}^t G^{[i]}Y_{t-i}\embed(M_{t-i})\in\mathbb{R}^{d_u+d_y}$, $\forall t$. Let $Y_t=\embed_y(y_{t-m+1:t}(K))$. Then, by \cref{eq:signal-obs}, we have
\begin{align*}
c_t(y_t,u_t)=c_t\left(B_t+\sum_{i=0}^{m-1} G^{[i]}Y_{t-i}\embed(M_{t-i})\right)=:f_t(\embed(M_{t-m+1}),\dots,\embed(M_t)),
\end{align*}
where $B_t$ is independent of $M_{t-m+1:t}$, and $Y_t$ is independent of $M_{1:T}$. We denote the unary form to be $\bar{f}_{t}$ as in \cref{def:induced-unary-form}
. Let $\mathcal{O}=\{\M(m,R_{\M}),m,\{f_t\}_{t\ge m,t\in\mathbb{N}}\}$ be the associated BCO-M instance (\cref{def:bco-m}).

By construction, $f_t$ satisfies \cref{asm:affine-memory} and \cref{asm:adv-adaptivity}. By assumption on $c_t$, the curvature assumption in \cref{asm:curvature} is also satisfied. It is left to check \cref{asm:regularity-bco-m}. 

\paragraph{Diameter bound on $\M(m,R_{\M})$.} The diameter of the set $\M(m,R_{\M})$ is given by
\begin{align*}
\max_{M_1,M_2\in\M(m,R_{\M})}\|\embed(M_1)-\embed(M_2)\|_2&\le \sqrt{m} \max_{M_1,M_2\in\M(m,R_{\M})}\max_{0\le j\le m-1}\|M_1^{[j]}-M_2^{[j]}\|_F\\
&\le \sqrt{m\max\{d_{u},d_{y}\}}\max_{M_1,M_2\in\M(m,R_{\M})}\max_{0\le j\le m-1}\|M_1^{[j]}-M_2^{[j]}\|_{\mathrm{op}}\\
&\le \sqrt{m\max\{d_{u},d_{y}\}} R_{\M}.
\end{align*}

\paragraph{Gradient bound of $f_t$.} By \cref{asm:strong-stabilizability} and the fact that $\forall M\in\mathbb{R}^{n\times n}$, $\|M\|_{\mathrm{op}}\le \sqrt{n}\|M\|_{\max}\le \sqrt{n}\|M\|_2$, we have that
\begin{align*}
\sum_{i=0}^{\infty}\|G^{[i]}\|_{\mathrm{op}}&\le 1+\sum_{i=1}^{\infty}\sqrt{\|C(A+BKC)^{i-1}B\|_{\mathrm{op}}^2+\|KC(A+BKC)^{i-1}B\|_{\mathrm{op}}^2}\\
&\le 1+\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2\sum_{i=1}^{\infty}\|HL^{i-1}H^{-1}\|_{2}\\
&\le 1+\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2\sum_{i=0}^{\infty} (1-\gamma)^i\\
&=1+\frac{\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2}{\gamma}.
\end{align*}

The signals $y_t(K)$ has the following norm bound:
\begin{align*}
\max_{t\in[T]}\|y_t(K)\|_2&=\max_{t\in[T]}\left\|C\sum_{i=0}^{t-1}(A+BKC)^iw_{t-i}+e_t\right\|_2\\
&\le R_{w,e}\left(1+\sqrt{d_x}\kappa_{\textbf{sys}}\sum_{i=1}^{\infty}\|HL^{i-1}H^{-1}\|_2\right)\\
&\le R_{w,e}\left(1+\frac{\sqrt{d_x}\kappa_{\textbf{sys}}}{\gamma}\right).
\end{align*}

By \cref{eq:signal-obs}, the observation and control pair $(y_t, u_t)$ has the following norm bound: $\forall t$,
\begin{align*}
\|(y_t, u_t)\|_2&\le \|(y_t(K),Ky_t(K))\|_2+\left\|\sum_{i=1}^t G^{[i]}\left(\sum_{j=0}^{m-1}M_{t-i}^{[j]}y_{t-i-j}(K)\right)\right\|_2\\
&\le R_{w,e}\left(1+\frac{\sqrt{d_x}\kappa_{\textbf{sys}}}{\gamma}\right)\left(\sqrt{1+\kappa^2}+R_{\M}\left\|\sum_{i=0}^{\infty}G^{[i]}\right\|_{\mathrm{op}}\right)\\
&\le R_{w,e}\left(1+\frac{\sqrt{d_x}\kappa_{\textbf{sys}}}{\gamma}\right)\left(\sqrt{1+\kappa^2}+R_{\M}\left(1+\frac{\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2}{\gamma}\right)\right).
\end{align*}

By the Lipschitz assumption on $c_t$, the gradient bound on $f_t$ is given by
\begin{align*}
& \quad \|\nabla f_t(\embed(M_{t-m+1}),\dots,\embed(M_{t}))\|_2\\
&= \left\|((G^{[m-1]}Y_{t-m+1})^{\top}\nabla c_t(y_t,u_t),\dots,(G^{[0]}Y_{t})^{\top}\nabla c_t(y_t,u_t)) \right\|_2\\
&\le \sqrt{m} \left(1+\frac{\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2}{\gamma}\right) G_c R_{w,e}^2\left(1+\frac{\sqrt{d_x}\kappa_{\textbf{sys}}}{\gamma}\right)^2\left(\sqrt{1+\kappa^2}+R_{\M}\left(1+\frac{\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2}{\gamma}\right)\right)^2\\
&\le \frac{4096\sqrt{m}G_cR_{w,e}^2R_{\M}^2d_x^{2.5}\kappa^3\kappa_{\textbf{sys}}^8}{\gamma^5}.
\end{align*}
$f_t$ is bounded over $\M(m,R_{\M})$ as
\begin{align*}
|f_t(\embed(M_{t-m+1}),\dots,\embed(M_{t}))|&= |c_t(y_t,u_t)|\\
&\le \beta_c \|(y_t,u_t)\|^2\\
&\le \beta_c R_{w,e}^2\left(1+\frac{\sqrt{d_x}\kappa_{\textbf{sys}}}{\gamma}\right)^2\left(\sqrt{1+\kappa^2}+R_{\M}\left(1+\frac{\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2}{\gamma}\right)\right)^2\\
&\le  \frac{1024\beta_c R_{w,e}^2R_{\M}^2d_x^2\kappa^2\kappa_{\textbf{sys}}^4}{\gamma^4}.
\end{align*}
Denote 
\begin{align*}
&\alpha_f=\alpha_c, \ \ \ \beta_f=\beta_c, \ \ \ D=\sqrt{m\max\{d_{u},d_{y}\}} R_{\M},\\
&G_f= \frac{4096\sqrt{m}G_cR_{w,e}^2R_{\M}^2d_x^{2.5}\kappa^3\kappa_{\textbf{sys}}^8}{\gamma^5}.
\end{align*}
We have that by \cref{asm:adversary} that
\begin{align*}
& \quad \E\left[\regret_T^{\A^{\mathrm{NC}}}(\ML)\right]\\
&=\max_{M\in\mathcal{M}(m,R_{\mathcal{M}})}\E\left[\sum_{t=1}^Tc_t(y_t(M_{1:t-1}),u_t(M_{1:t-1}))-c_t(y_t(M),u_t(M))\right]\\
&\le G_fDm+\E\left[\sum_{t=m}^Tf_t(\embed(M_{t-m+1}),\dots,\embed(M_t))-\bar{f}_t(\embed(M))\right]\\
& \quad +\E\left[\sum_{t=m}^T\bar{f}_t(\embed(M))-c_t(y_t(M),u_t(M))\right]\\
&=\E\left[\sum_{t=m}^Tc_t\left(B_t+\sum_{i=0}^{m-1} G^{[i]}Y_{t-i}\embed(M))\right)-c_t\left((y_t(K), Ky_t(K))+\sum_{i=0}^{t}G^{[i]}Y_{t-i}\embed(M)\right)\right]\\
& \quad +\E\left[\sum_{t=m}^Tf_t(\embed(M_{t-m+1}),\dots,\embed(M_t))-\bar{f}_t(\embed(M))\right]+ G_fDm,
\end{align*}
where we have
\begin{align*}
& \quad c_t\left(B_t+\sum_{i=0}^{m-1} G^{[i]}Y_{t-i}\embed(M))\right)-c_t\left((y_t(K), Ky_t(K))+\sum_{i=0}^{t}G^{[i]}Y_{t-i}\embed(M)\right)\\
& \le G_c\left\|\sum_{i=m}^t G^{[i]}Y_{t-i}\embed(M)\right\|_2\le G_c\sum_{i=m}^t \|G^{[i]}\|_{\mathrm{op}}\|Y_{t-i}\|_F \|M\|_F.
\end{align*}
Recall that
\begin{align*}
\|M\|_F^2&=\sum_{j=0}^{m-1}\|M^{[j]}\|_F^2\le \max\{d_u,d_y\}\sum_{j=0}^{m-1}\|M^{[j]}\|_{\mathrm{op}}^2\le m\max\{d_u,d_y\}R_{\M}^2,\\
\max_{t\in[T]}\|Y_t\|_2&=\sqrt{md_yd_u^2}\cdot\max_{t\in[T]}\|y_t(K)\|_2\le \sqrt{md_yd_u^2}\cdot R_{w,e}\left(1+\frac{\sqrt{d_x}\kappa_{\textbf{sys}}}{\gamma}\right),\\
\sum_{i=m}^{\infty}\|G^{[i]}\|_{\mathrm{op}}&\le \sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2\sum_{i=m}^{\infty}(1-\gamma)^i\le\frac{\sqrt{d_x(1+\kappa^2)}\kappa_{\textbf{sys}}^2(1-\gamma)^m}{\gamma}.
\end{align*}
We have for $m=\Theta\left(\log T/\log(1/(1-\gamma))\right)$, 
\begin{align*}
G_c\sum_{i=m}^t \|G^{[i]}\|_{\mathrm{op}}\|Y_{t-i}\|_F \|M\|_F&\le \frac{2G_cmd_yd_u^2 d_x(1+\kappa^2)\kappa_{\textbf{sys}}^4R_{\M}(1-\gamma)^m}{\gamma^2}\\
&\le \frac{G_cmd_yd_u^2 d_x\kappa^2\kappa_{\textbf{sys}}^4R_{\M}}{\gamma^2T}.
\end{align*}
Combining, we have
\begin{align*}
\E\left[\regret_T^{\A^{\mathrm{NC}}}(\ML)\right]&\le \E\left[\regret_T^{\A^{\mathrm{B}}}(\mathcal{O})\right]+\frac{G_cmd_yd_u^2 d_x\kappa^2\kappa_{\textbf{sys}}^4R_{\M}}{\gamma^2}+G_fDm\\
&\le \E\left[\regret_T^{\A^{\mathrm{B}}}(\mathcal{O})\right]+2G_fDm,
\end{align*}
which concludes the claim that $\mathcal{O}$ $2G_fDmT^{-1}$-approximates $\ML$. 
\end{proof}

==> check.tex <==
\section*{NeurIPS Paper Checklist}


 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we make sure all the claims are accurate.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we discuss the limitations and future directions for improvement in the Discussion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we provide the full set of assumptions for all theoretical results. We provide a complete (and correct) proof to for all theoretical results, among which the simpler ones are left to the appendix.
    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: paper does not include experiments requiring code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we carefully follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: there is no societal impact of the work performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not use existing assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
